How Computers Work: Computational Thinking for Everyone

What would you teach if you had only one course to help students grasp the essence of computation and perhaps inspire a few of them to make computing a subject of further study? Assume they have the standard college prep background. This would include basic algebra, but not necessarily more advanced mathematics. They would have written a few term papers, but would not have written computer programs. They could surf and twitter, but could not exclusive-or and nand. What about computers would interest them or help them place their experience in context? This paper provides one possible answer to this question by discussing a course that has completed its second iteration. Grounded in classical logic, elucidated in digital circuits and computer software, it expands into areas such as CPU components and massive databases. The course has succeeded in garnering the enthusiastic attention of students with a broad range of interests, exercising their problem solving skills, and introducing them to computational thinking.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{M. Moraz\'an and P. Achten (Eds.): Trends in Functional \\ Programming in Education 2012 (TFPIE 2012).\\
EPTCS 106, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.106.1}{10.4204/EPTCS.106.1}}

